Efficient analysis of caching strategies under dynamic content popularity

In this paper we develop a novel technique to analyze both isolated and interconnected caches operating under different caching strategies and realistic traffic conditions. The main strength of our approach is the ability to consider dynamic contents which are constantly added into the system catalogue, and whose popularity evolves over time according to desired profiles. We do so while preserving the simplicity and computational efficiency of models developed under stationary popularity conditions, which are needed to analyze several caching strategies. Our main achievement is to show that the impact of content popularity dynamics on cache performance can be effectively captured into an analytical model based on a fixed content catalogue (i.e., a catalogue whose size and objects' popularity do not change over time).

==> preliminaries.tex <==
\section{System assumptions}\label{sec:prelim}

We start introducing some notation and assumptions.
In the simplest case, there is only one cache, whose size, expressed
in number of \lq objects', is denoted by $C$. 

%Note that the storage capacity of a cache is typically measured 
%in bytes, rather than objects, however in the modelling literature it is 
%common to express it in number of objects or items, to avoid 
%the additional complexity related to heterogeneous object sizes.
%However, this assumption is not particularly restrictive, 
%since we can always split the objects into constant-size pieces 
%(e.g., chunks) and reason in terms of such pieces (in the extreme case,
%individual bytes).

The cache is fed by an exogenous arrival process of objects' requests
generated by users. Requests which find the object in the cache
are said to produce a \textit{hit}, whereas requests that do not find the object in 
the cache are said to produce a \textit{miss}. The main performance metric of interest
is the \textit{hit probability}, which is the fraction of requests producing a hit. 

In the case of cache networks, the \textit{miss stream} of a cache, i.e., the
process of requests which are not locally satisfied by the cache,
is forwarded to one or more caches (deterministically or at random), 
or to a common repository  storing entire object catalogue.
Eventually, all requests hit the target, and it is common in the modelling 
literature to neglect all propagation delays, 
%i.e., the effects produced in the network by a request occur in negligible time (before the arrival of the next request), 
including the delays necessary to 
possibly insert the object in one or more caches not storing it, in response to a miss. 

Cache systems and their analysis can be distinguished on the basis
of three main ingredients: i) the traffic model, i.e., the stochastic characterization 
of the request process generated by users; ii) the cache policy, i.e., 
how an individual cache reacts to a given object request; iii) the replication strategy,
i.e., how the entire cache network reacts to an object request, deciding in particular
in which caches objects get replicated back after a request hits the target.
We separately discuss each of the above ingredients in the next sections.

\subsection{Traffic models}\label{subsec:traffic}
We first recall the so-called Independent Reference Model (IRM), which
is de-facto the standard approach adopted in the literature to 
characterize the pattern of object requests arriving at a cache \cite{Coffman:73}. 
The IRM is based on the following fundamental assumptions: i) users request items
from a fixed catalogue of $M$ object; 
%ii) the probability $p_m$ that a request is for object 
%$m$, \mbox{$1 \leq m \leq M$}, is constant (\emph{i.e.}, the object popularity does not vary over time)
%and {\em independent} of all past requests, generating an i.i.d. sequence of requests.
ii)  the process of requests of a given object is modeled by  a homogeneous Poisson process of intensity $\lambda_m = \Lambda p_m$.

The IRM is commonly used in combination with a Zipf-like law of probability $p_m$, 
which is the typical object popularity distribution observed in traffic measurements and widely adopted in
performance evaluation studies~\cite{zipf,Roberts_mix}.

%In its simplest form, Zipf's law states that the probability to request the $i$-th
%most popular item is proportional to $1/i^\alpha$, where the exponent
%$\alpha$ depends on the considered system (especially on the type of
%objects)~\cite{Roberts_mix}, and plays a crucial role on the resulting 
%cache performance. Estimates of $\alpha$ reported in the 
%literature for various kinds of systems range between .65 and 1.

%One way to generate an arrival process of requests satisfying the assumptions of IRM
%is the following: let $\Lambda$ be the aggregate arrival rate of requests; the requests
%for a given object $m$ are generated, independently of all other objects, according
%to a homogeneous Poisson process of intensity $\lambda_m = \Lambda p_m$;
%then we superpose over time the obtained processes related to individual objects.  
%Standard properties of Poisson processes guarantee that the aggregate sequence
%of contents' requests is i.i.d. with the desired popularity distribution.

By definition, the IRM completely ignores all temporal correlations 
in the sequence of requests. In particular, it does not take into account 
a key feature of real traffic usually referred to as {\em temporal locality},
i.e., the fact that, if an object is requested at a given point in time, 
then it is more likely that the same object will be requested again in the near future.
It is well known that traffic locality has a beneficial effect on cache performance
(i.e., it increases the hit probability)~\cite{Coffman:73} and several 
extensions of IRM have been proposed to incorporate it into a traffic model.
Existing approaches \cite{Coffman:73,virtamo98,amiciburini} 
typically assume that the request process for each object is 
stationary (i.e., either a renewal process or a Markov- or semi-Markov-modulated 
Poisson process).

One simple way to incorporate traffic locality in the traffic is the following.
Instead of a standard Poisson process (which produces an IRM sequence, as already said), 
the request process for a certain content at an ingress cache is described by an independent renewal process
with given inter-request time distribution. Let $F_R(m,t)$ be the cdf of the inter-request 
time $t$ for object $m$. The average request rate $\lambda_m$ for content $m$, which can be
expressed by $\lambda_m = 1/\int_0^\infty(1-F_R(m,t)) \diff t$, matches 
the desired average rate $\lambda_m = \Lambda p_m$. 
In the following, we will refer to the above traffic model as {\em renewal} traffic. 
As we will later see, these assumptions are not really 
appropriate to capture the kind of temporal locality usually
encountered in Video-on-Demand traffic,
%related to content
%distribution systems such as Video-on-Demand,
because they cannot easily capture macroscopic, intrinsically
non-stationary effects related to content popularity dynamics.

Recently \cite{TraversoCCR} a new traffic model, named Shot Noise Model (SNM)
has been proposed as a viable alternative to traditional traffic models to capture macroscopic
effects related to content popularity dynamics. The  basic idea of the SNM is  to represent the overall request process as the superposition of many independent processes (shots), each referring to an
individual content. Specifically, the arrival process of requests for 
a given content $m$ at a cache is described by an inhomogeneous Poisson process of intensity 
$V_m h(t-t_m)$, where $V_m$ denotes the average number of requests attracted by the content,
$t_m$ is the time instant at which the content enters the
system (i.e., it becomes available to the users), and $h()$ 
is the (normalized) ``popularity profile'' of content $m$. 

SNM has been shown in~\cite{TraversoCCR} to provide a simple, flexible and accurate approach
to describing the temporal and geographical locality found in Video-on-Demand traffic.  
An interesting finding in~\cite{TraversoCCR} is that the particular shape of the
``popularity profile'' $h()$ has very little impact on the cache performance,
which essentially depends only on the average content life-span $L$.
This property actually plays a crucial role in our analytical methodology, as we will see.

To illustrate these facts, Figure~\ref{fig:figures/phit_vs_cachesize_fertility_flip_trace_04} reports 
the cache size needed to achieve a desired hitting probability in a LRU cache fed by a real 
trace of YouTube video requests, which was kindly provided to us by the authors of~\cite{TraversoCCR}.
The trace was fitted by a multiclass SNM traffic model with 4 classes, 
all of them sharing the same shape for the ``popularity profile'' (but with different average life-span).
Results in Fig.~\ref{fig:figures/phit_vs_cachesize_fertility_flip_trace_04} 
show that rather different shapes for the SNM (e.g., uniform vs power-law) produce
very similar curves, both in good agreement with results derived 
under the original Youtube trace. The curve labelled ON-OFF, also very close to 
the trace, can be obtained by adopting the methodology described in this paper, as explained later.
The plot contains also a curve labelled 'Naive IRM', corresponding to the cache performance 
observed after the application of a random permutation to the requests contained in the original trace: by so doing, 
the temporal locality present in the original trace is washed out, allowing us to assess 
the prediction error that one would get by following a naive IRM approach. 

\tgifeps{7.0}{figures/phit_vs_cachesize_fertility_flip_trace_04}{Hit probability vs cache size, resulting from
feeding an LRU cache by: the original YouTube trace, a fitted multi-class SNM, our ON-OFF traffic model, and 
a reshuffled trace analogous to a naive application of the IRM model.}

\subsection{Cache policies} \label{subsec:policy}
In this work we will focus on the following strategies controlling the
behavior of an individual cache:
\begin{itemize}
\item {\bf LRU}: upon arrival of a request, an object not already stored in the cache is inserted into it.
If the cache is full, to make room for a new object the {\em Least Recently Used} item is evicted, i.e., the
object which has not been requested for the longest time.
\item {\bf q-LRU}: it differs from LRU for the insertion policy: upon arrival of a request, 
an object not already stored in the cache is inserted into it with probability $q$. 
% The eviction policy is the same as LRU.
\item{\bf RANDOM}:  it differs from LRU for the eviction policy: 
to make room for a new object, a random item stored in the cache is evicted.
\item{\bf 2-LRU}: this strategy, proposed in \cite{nostro_infocom}, is based on an 
effective, self-tuning insertion policy working as follows:
before arriving at the physical cache (storing actual objects),
requests have to traverse a virtual LRU cache put in front of it, 
which stores just object ID's. Only requests for objects whose ID is found in the 
virtual cache are forwarded to the physical cache.
The eviction policy at both caches, which for simplicity are assumed to be of the same size
(expressed either in terms of objects or ID's) is like LRU.  
\end{itemize}

%We remark that LRU has been widely adopted, since it provides good performance while 
%being reasonably simple to implement. RANDOM has been considered as 
%viable alternative to LRU in the context of ICN, as its hardware implementation
%in high-speed routers is even simpler. The performance of RANDOM is similar to LRU,
%since the insertion policy is the same, while the eviction policy is known to have
%marginal impact on cache performance.

%The performance of LRU (or RANDOM), instead, can be significantly improved by means of
%better insertion policies \cite{jel08}, which try to avoid the insertion of objects which are
%not likely to be requested again in the near future (i.e., within the cache eviction time).
%We have chosen q-LRU in light of its simplicity, and the 
%fact that it can be given an immediate interpretation 
%in terms of probabilistic replication for cache networks (see next section).

\subsection{Replication strategies for cache networks}\label{subsec:rep}
In a system of interconnected caches, we need to specify
what happens along the route traversed by a request, after
the request eventually hits the target (in the worst case, ending up
at the repository containing all objects).  

We will consider the following mechanisms:
\begin{itemize}
\item {\bf leave-copy-everywhere (LCE)}: the object is 
put into all caches of the backward path.
\item {\bf leave-copy-probabilistically (LCP)}: the object is put with 
probability $q$ into each cache of the backward path.
%\item {\bf leave-copy-down (LCD)}: the object is sent only to the 
%cache preceding the one in which the object is found (if any).
\end{itemize}
An important property is the following: if we combine the LCP
replication strategy with standard LRU policy at all caches,
we obtain a cache system analogous to the one in which we adopt 
LCE replication in combination with q-LRU at all caches.
Hence, developing a model of q-LRU for individual caches
permits analysing LCP in a straightforward way.

We will not analyse in this work the leave-copy-down (LCD)
replication strategy, according to which the object is replicated only 
in the cache preceding the one in which it is found (if this is not an ingress cache). 
This would be an interesting direction of future research, in light of the 
excellent performance exhibited by this policy, which is
however more complex to analyze \cite{lao06}.

\begin{comment}
\subsection{The Che approximation} \label{subsec:che-approx}
We briefly recall here the Che's approximation for LRU  under the classical
IRM \cite{che}. 
% We define the {\em cache eviction time} for content $m$ as the time
% interval from last request for content $m$ after which content $m$
% is evicted from the cache.  Che's approximation consists in assuming
% the {\em cache eviction time} to be both deterministic and invariant
% with respect to the specific content.
Consider a cache capable of storing $C$ distinct objects. Let
$T_C(m)$ be the time needed before $C$ distinct objects (not including
$m$) are requested by users. Therefore, $T_C(m)$ is the {\em
cache eviction time} for content $m$, i.e., the time since the last request after 
which object $m$ will be evicted from the cache (if the object is not again requested 
in the meantime).  

Che's approximation assumes $T_C(m)$ to be
a constant independent of the selected content $m$.
This assumption has been given a theoretical justification in~\cite{Roberts1}, where it is
shown that, under a Zipf-like popularity distribution, the
coefficient of variation of the random variable representing $T_C(m)$
tends to vanish as the cache size grows. Furthermore, the dependence
of the eviction time on $m$ becomes negligible when the catalogue size 
is sufficiently large.  

The reason why Che's approximation greatly simplifies the analysis of 
caching systems is because it allows to decouple 
the dynamics of different contents: interaction among the 
contents is summarized by $T_C$, which acts as a single 
primitive quantity representing the response of the cache
to an object request.

%The arguments given
%in~\cite{Roberts1} are easily extended to our non-stationary traffic
%model when $\gamma$ and $C$ are sufficiently large.
%In ~\cite{Roberts1} authors also discover that
%Che's approximation is surprisingly accurate also in critical cases (small catalogue,
%very uneven popularity law). 

More in detail, thanks to Che's approximation, we can state that 
an object $m$ is in the cache at time $t$, if and only if a time
smaller than $T_C$ has elapsed since the last request for object $m$,
i.e., if at least a request for $m$ has arrived in the
interval $(t-T_c,t]$. Under the assumption that requests for object $m$ arrive according 
to a Poisson process of rate $\lambda_m$, 
the time-average probability $p_{\text{in}}(m)$ that object $m$ 
is in the cache is given by:  
\begin{equation}\label{eq:phm}
p_{\text{in}}(m) = 1- e^{-\lambda_{m} T_c} 
\end{equation}
As immediate consequence of PASTA property for Poisson arrivals, 
observe that $p_{\text{in}}(m)$ represents, by construction, 
also the hit probability $p_{\text{hit}}(m)$,  i.e., the probability that a 
request for object $m$ finds object $m$ in the cache.   

Considering a cache of size $C$, by construction: 
\[ 
C= \sum_{m} \Uno_{\{\text{$m$ in cache}\}} 
\]
After averaging both sides, we obtain:
\be\label{eq:C}
C= \sum_{m} \mathbb{E}[\Uno_{\{\text{$m$ in cache}\}} ]= \sum_m p_{\text{in}}(m).
\ee
The only unknown quantity in the above equality is $T_C$,
which can be obtained with arbitrary precision by a fixed point procedure.
% By solving the above eqfirst order moment matching equation, we obtain $T_c$, and 
The average hit probability of the cache is then:
\begin{equation}\label{eq:phmtot}
p_{\text{hit}}= \sum_{m} p_m \, p_{\text{hit}}(m)
\end{equation}
% with $p_{mc}= \lambda_{m}/\sum_{m'}\lambda_{m'}$.
% with $p_m= \lambda_m/\Lambda$

%The  reason why   Che's approximation allows to greatly simplify the analysis of caching systems is because
%it allows us to decouple the  dynamics of different contents, making essentially the behavior of each individual content  independent, given 
%$T_C$.  the eviction time $T_C$  that  must be numerically evaluated, summarizes  the  dynamic interdependency  among contents different contents



%whose stochastic characterization is a priori given,  can be generalized 
% to other caching strategies, under more general traffic models. This provides
% a very powerful tool to predict  the performance and to show properties
%of caches and networks of caches.

\end{comment}


